Partition of Unity Extension of Functions on Complex Domains

We introduce an efficient algorithm, called partition of unity extension or PUX, to construct an extension of desired regularity of a function given on a complex multiply connected domain in $2D$. Function extension plays a fundamental role in extending the applicability of boundary integral methods to inhomogeneous partial differential equations with embedded domain techniques. Overlapping partitions are placed along the boundaries, and a local extension of the function is computed on each patch using smooth radial basis functions; a trivially parallel process. A partition of unity method blends the local extrapolations into a global one, where weight functions impose compact support. The regularity of the extended function can be controlled by the construction of the partition of unity function. We evaluate the performance of the PUX method in the context of solving the Poisson equation on multiply connected domains using a boundary integral method and a spectral solver. With a suitable choice of parameters the error converges as a tenth order method down to $10^{-14}$.

==> sections/comments.tex <==
\begin{itemize}
\item The Poisson equation, not Poisson's equation
\item Acronyms in use: FFT, FMM, GMRES, PDE, RBF, RPF-QR, PUX
\item I do not comment how much time constructing and solving the free-space Poissons equation takes. Reason: Some parts of the code (for solving Poisson on complex domain) are optimized, some are not.
\item Typesetting of images is not done.
\item Let uniform points, or evaluation points be $y$

\item Can I call the function extension "high regularity"? We use least squares so it is discontinuous. 

\end{itemize}

% \newpage
% \begin{itemize}
% \item $w$: partition of unity weight function
% \item $u$: solution to Poissons equation
% \item $u^{P}$: particular solution to Poissons equation
% \item $u^{H}$: homogeneuous solution to Poissons equation
% \item $g$: given boundary conditions for Poissons equation
% \item $\tilde{g}$: modified boundary conditions for homogeneuous Poissons equation
% \item $f$: given right hand side for Poissons equation
% \item $f^e$: function extension of $f$
% \item $\mu$: double layer density
% \item $\Omega$: domain on which $f$ is given
% \item $\Omega_i$: patch correpsonding to one partition
% \item $N$: number of partitions
% \item $M$: number of RBF--centres.
% \item $M_{i}$: number of RBF--centres for partition $\Omega_{i}$
% \item $\lambda_{j}$: partition weight
% \item $j$: index for RBF
% \item $i$: index for partitions
% \item $\varphi$: RBF
% \item $N^{0}$: number of zero--partitions
% \item $\Omega^{e}$: Set difference between domain embedding $\Omega$ and $\Omega$
% \end{itemize}
% \newpage
